MirrorCalib: Utilizing Human Pose Information for Mirror-based Virtual Camera Calibration

In this paper, we present the novel task of estimating the extrinsic parameters of a virtual camera relative to a real camera in exercise videos with a mirror. This task poses a significant challenge in scenarios where the views from the real and mirrored cameras have no overlap or share salient features. To address this issue, prior knowledge of a human body and 2D joint locations are utilized to estimate the camera extrinsic parameters when a person is in front of a mirror. We devise a modified eight-point algorithm to obtain an initial estimation from 2D joint locations. The 2D joint locations are then refined subject to human body constraints. Finally, a RANSAC algorithm is employed to remove outliers by comparing their epipolar distances to a predetermined threshold. MirrorCalib achieves a rotation error of 1.82{\deg} and a translation error of 69.51 mm on a collected real-world dataset, which outperforms the state-of-art method.

==> egbib.tex <==
@InProceedings{b1,
author="Rodrigues, Rui
and Barreto, Jo{\~a}o P.
and Nunes, Urbano",
editor="Daniilidis, Kostas
and Maragos, Petros
and Paragios, Nikos",
title="Camera Pose Estimation Using Images of Planar Mirror Reflections",
booktitle="Computer Vision -- ECCV 2010",
year="2010",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="382--395",
abstract="The image of a planar mirror reflection (IPMR) can be interpreted as a virtual view of the scene, acquired by a camera with a pose symmetric to the pose of the real camera with respect to the mirror plane. The epipolar geometry of virtual views associated with different IPMRs is well understood, and it is possible to recover the camera motion and perform 3D scene reconstruction by applying standard structure-from-motion methods that use image correspondences as input. In this article we address the problem of estimating the pose of the real camera, as well as the positions of the mirror plane, by assuming that the rigid motion between N virtual views induced by planar mirror reflections is known. The solution of this problem enables the registration of objects lying outside the camera field-of-view, which can have important applications in domains like non-overlapping camera network calibration and robot vision. We show that the positions of the mirror planes can be uniquely determined by solving a system of linear equations. This enables to estimate the pose of the real camera in a straightforward closed-form manner using a minimum of N{\thinspace}={\thinspace}3 virtual views. Both synthetic tests and real experiments show the superiority of our approach with respect to current state-of-the-art methods.",
isbn="978-3-642-15561-1"
}
@INPROCEEDINGS{b2,
  author={Takahashi, Kosuke and Nobuhara, Shohei and Matsuyama, Takashi},
  booktitle={2012 IEEE Conference on Computer Vision and Pattern Recognition}, 
  title={A new mirror-based extrinsic camera calibration using an orthogonality constraint}, 
  year={2012},
  volume={},
  number={},
  pages={1051-1058},
  keywords={Mirrors;Cameras;Vectors;Calibration;Eigenvalues and eigenfunctions;Equations;Mathematical model},
  doi={10.1109/CVPR.2012.6247783}}

@INPROCEEDINGS{b3,
  author={Kumar, Ram Krishan and Ilie, Adrian and Frahm, Jan-Michael and Pollefeys, Marc},
  booktitle={2008 IEEE Conference on Computer Vision and Pattern Recognition}, 
  title={Simple calibration of non-overlapping cameras with a mirror}, 
  year={2008},
  volume={},
  number={},
  pages={1-7},
  keywords={Calibration;Cameras;Mirrors;Computer vision;Computer science;Application software;Nonlinear distortion;Parameter estimation;Image reconstruction;Motion estimation},
  doi={10.1109/CVPR.2008.4587676}}

@INPROCEEDINGS{b4,
  author={Gucan Long and Kneip, Laurent and Xin Li and Xiaohu Zhang and Qifeng Yu},
  booktitle={2015 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Simplified mirror-based camera pose computation via rotation averaging}, 
  year={2015},
  volume={},
  number={},
  pages={1247-1255},
  keywords={Cameras;Mirrors;Transmission line matrix methods;Calibration;Three-dimensional displays},
  doi={10.1109/CVPR.2015.7298729}}

@INPROCEEDINGS{b5,
  author={Agrawal, Amit and Ramalingam, Srikumar},
  booktitle={2013 IEEE Conference on Computer Vision and Pattern Recognition}, 
  title={Single Image Calibration of Multi-axial Imaging Systems}, 
  year={2013},
  volume={},
  number={},
  pages={1399-1406},
  keywords={Mirrors;Cameras;Calibration;Equations;Estimation;Noise;calibration;catadioptric;spherical mirror;wide-angle;axial},
  doi={10.1109/CVPR.2013.184}}

@INPROCEEDINGS{b6,
  author={Nene, S.A. and Nayar, S.K.},
  booktitle={Sixth International Conference on Computer Vision (IEEE Cat. No.98CH36271)}, 
  title={Stereo with mirrors}, 
  year={1998},
  volume={},
  number={},
  pages={1087-1094},
  keywords={Mirrors;Cameras;Layout;Lenses;Calibration;Three dimensional displays;Optical refraction;Computer science;Optical imaging;Rendering (computer graphics)},
  doi={10.1109/ICCV.1998.710852}}

@article{b7,
author = {Gluckman, Joshua and Nayar, Shree},
year = {2001},
month = {08},
pages = {65-79},
title = {Catadioptric Stereo Using Planar Mirrors},
volume = {44},
journal = {International Journal of Computer Vision},
doi = {10.1023/A:1011172403203}
}
@INPROCEEDINGS{b8,
  author={Tahara, Tomu and Kawahara, Ryo and Nobuhara, Shohei and Matsuyama, Takashi},
  booktitle={2015 International Conference on 3D Vision}, 
  title={Interference-Free Epipole-Centered Structured Light Pattern for Mirror-Based Multi-view Active Stereo}, 
  year={2015},
  volume={},
  number={},
  pages={153-161},
  keywords={Mirrors;Three-dimensional displays;Cameras;Geometry;Lighting;Shape;Sensors;3D shape capture;Structured-light;Mirror},
  doi={10.1109/3DV.2015.25}}

@article{b9,
title = {Surround structured lighting: 3-D scanning with orthographic illumination},
journal = {Computer Vision and Image Understanding},
volume = {113},
number = {11},
pages = {1107-1117},
year = {2009},
note = {Special issue on New Advances in 3D Imaging and Modeling},
issn = {1077-3142},
doi = {https://doi.org/10.1016/j.cviu.2009.03.016},
url = {https://www.sciencedirect.com/science/article/pii/S1077314209000721},
author = {Douglas Lanman and Daniel Crispell and Gabriel Taubin},
keywords = {3-D reconstruction, Structured lighting, Gray codes, Orthographic projection, Full object scanning},
abstract = {This paper presents a new system for rapidly acquiring complete 3-D surface models using a single orthographic structured light projector, a pair of planar mirrors, and one or more synchronized cameras. Using the mirrors, we project structured light patterns that illuminate the object from all sides (not just the side of the projector) and are able to observe the object from several vantage points simultaneously. This system requires that projected planes of light to be parallel, so we construct an orthographic projector using a Fresnel lens and a commercial DLP projector. A single Gray code sequence is used to encode a set of vertically-spaced light planes within the scanning volume, and five views of the illuminated object are obtained from a single image of the planar mirrors located behind it. From each real and virtual camera we recover a dense 3-D point cloud spanning the entire object surface using traditional structured light algorithms. A key benefit of this design is to ensure that each point on the object surface can be assigned an unambiguous Gray code sequence, despite the possibility of being illuminated from multiple directions. In addition to presenting a prototype implementation, we also develop a complete set of mechanical alignment and calibration procedures for utilizing orthographic projectors in computer vision applications. As we demonstrate, the proposed system overcomes a major hurdle to achieving full 360° reconstructions using a single structured light sequence by eliminating the need for merging multiple scans or multiplexing several projectors.}
}
@article{b10,
  title={Self-Calibration of Catadioptric Camera with Two Planar Mirrors from Silhouettes},
  author={Xianghua Ying and Kun Peng and Yongbo Hou and Sheng Guan and Jing Kong and Hongbin Zha},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2013},
  volume={35},
  pages={1206-1220},
  url={https://api.semanticscholar.org/CorpusID:8578265}
}
@InProceedings{b11,
author="Puwein, Jens
and Ballan, Luca
and Ziegler, Remo
and Pollefeys, Marc",
editor="Cremers, Daniel
and Reid, Ian
and Saito, Hideo
and Yang, Ming-Hsuan",
title="Joint Camera Pose Estimation and 3D Human Pose Estimation in a Multi-camera Setup",
booktitle="Computer Vision -- ACCV 2014",
year="2015",
publisher="Springer International Publishing",
address="Cham",
pages="473--487",
abstract="In this paper we propose an approach to jointly perform camera pose estimation and human pose estimation from videos recorded by a set of cameras separated by wide baselines. Multi-camera pose estimation is very challenging in case of wide baselines or in general when patch-based feature correspondences are difficult to establish across images.",
isbn="978-3-319-16808-1"
}
@INPROCEEDINGS{b12,
  author={Takahashi, Kosuke and Mikami, Dan and Isogawa, Mariko and Kimata, Hideaki},
  booktitle={2018 IEEE/CVF Conference on Computer Vision and Pattern Recognition Workshops (CVPRW)}, 
  title={Human Pose as Calibration Pattern: 3D Human Pose Estimation with Multiple Unsynchronized and Uncalibrated Cameras}, 
  year={2018},
  volume={},
  number={},
  pages={1856-18567},
  doi={10.1109/CVPRW.2018.00230}}
@INPROCEEDINGS{b13,
  author={Huang, Buzhen and Shu, Yuan and Zhang, Tianshu and Wang, Yangang},
  booktitle={2021 International Conference on 3D Vision (3DV)}, 
  title={Dynamic Multi-Person Mesh Recovery From Uncalibrated Multi-View Cameras}, 
  year={2021},
  volume={},
  number={},
  pages={710-720},
  keywords={Geometry;Three-dimensional displays;Semantics;Dynamics;Cameras;Calibration;Noise measurement;Human mesh recovery;Extrinsic camera calibration;Motion prior},
  doi={10.1109/3DV53792.2021.00080}}

@inproceedings{b14,
author = {Ben-Artzi, Gil and Kasten, Yoni and Peleg, Shmuel and Werman, Michael},
year = {2016},
month = {06},
pages = {4095-4103},
title = {Camera Calibration from Dynamic Silhouettes Using Motion Barcodes},
doi = {10.1109/CVPR.2016.444}
}
@article{b15,
author = {Sinha, Sudipta and Pollefeys, Marc},
year = {2010},
month = {05},
pages = {266-283},
title = {Camera Network Calibration and Synchronization from Silhouettes in Archived Video},
volume = {87},
journal = {International Journal of Computer Vision},
doi = {10.1007/s11263-009-0269-2}
}
@article{b16,
title = {Planar mirrors for image-based robot localization and 3-D reconstruction},
journal = {Mechatronics},
volume = {22},
number = {4},
pages = {398-409},
year = {2012},
note = {Visual Servoing SI},
issn = {0957-4158},
doi = {https://doi.org/10.1016/j.mechatronics.2011.09.004},
url = {https://www.sciencedirect.com/science/article/pii/S0957415811001474},
author = {Gian Luca Mariottini and Stefano Scheggi and Fabio Morbidi and Domenico Prattichizzo},
keywords = {Robot vision systems, Catadioptric sensor, Stereo vision, Eye-in-hand robot},
abstract = {Planar catadioptric vision sensors consist of a pinhole camera observing a scene being reflected on two (or more) planar mirrors. These systems have recently received an increasing attention because, unlike stereo cameras, can capture two views of the same scene without the need of hardware multi-camera synchronization and calibration. In this paper we explore the original scenario in which a robot manipulator, equipped with a pinhole camera on its end-effector, observes an unknown 3-D scene both directly and reflected through multiple mirrors. We present new multiple-view properties for this scenario and, based on these theoretical results, we present new image-based camera localization and new 3-D scene reconstruction algorithms. Extensive simulation and real-data experiments illustrate the theory and show the effectiveness of the proposed designs.}
}
@ARTICLE{b17,
  author={Hartley, R.I.},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
  title={In defense of the eight-point algorithm}, 
  year={1997},
  volume={19},
  number={6},
  pages={580-593},
  keywords={Iterative algorithms;Layout;Cameras;Equations;Image reconstruction;Algorithm design and analysis;Stereo vision;Computer vision;Least squares methods},
  doi={10.1109/34.601246}}

@ARTICLE {b18,
author = {J. Wang and K. Sun and T. Cheng and B. Jiang and C. Deng and Y. Zhao and D. Liu and Y. Mu and M. Tan and X. Wang and W. Liu and B. Xiao},
journal = {IEEE Transactions on Pattern Analysis &amp; Machine Intelligence},
title = {Deep High-Resolution Representation Learning for Visual Recognition},
year = {2021},
volume = {43},
number = {10},
issn = {1939-3539},
pages = {3349-3364},
abstract = {High-resolution representations are essential for position-sensitive vision problems, such as human pose estimation, semantic segmentation, and object detection. Existing state-of-the-art frameworks first encode the input image as a low-resolution representation through a subnetwork that is formed by connecting high-to-low resolution convolutions in series (e.g., ResNet, VGGNet), and then recover the high-resolution representation from the encoded low-resolution representation. Instead, our proposed network, named as High-Resolution Network (HRNet), maintains high-resolution representations through the whole process. There are two key characteristics: (i) Connect the high-to-low resolution convolution streams in parallel and (ii) repeatedly exchange the information across resolutions. The benefit is that the resulting representation is semantically richer and spatially more precise. We show the superiority of the proposed HRNet in a wide range of applications, including human pose estimation, semantic segmentation, and object detection, suggesting that the HRNet is a stronger backbone for computer vision problems. All the codes are available at https://github.com/HRNet.},
keywords = {spatial resolution;semantics;object detection;pose estimation;convolutional codes;indexes;image segmentation},
doi = {10.1109/TPAMI.2020.2983686},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month = {oct}
}

BibTeX
@article{b19,
author = {Loper, Matthew and Mahmood, Naureen and Romero, Javier and Pons-Moll, Gerard and Black, Michael J.},
title = {SMPL: a skinned multi-person linear model},
year = {2015},
issue_date = {November 2015},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {34},
number = {6},
issn = {0730-0301},
url = {https://doi.org/10.1145/2816795.2818013},
doi = {10.1145/2816795.2818013},
abstract = {We present a learned model of human body shape and pose-dependent shape variation that is more accurate than previous models and is compatible with existing graphics pipelines. Our Skinned Multi-Person Linear model (SMPL) is a skinned vertex-based model that accurately represents a wide variety of body shapes in natural human poses. The parameters of the model are learned from data including the rest pose template, blend weights, pose-dependent blend shapes, identity-dependent blend shapes, and a regressor from vertices to joint locations. Unlike previous models, the pose-dependent blend shapes are a linear function of the elements of the pose rotation matrices. This simple formulation enables training the entire model from a relatively large number of aligned 3D meshes of different people in different poses. We quantitatively evaluate variants of SMPL using linear or dual-quaternion blend skinning and show that both are more accurate than a Blend-SCAPE model trained on the same data. We also extend SMPL to realistically model dynamic soft-tissue deformations. Because it is based on blend skinning, SMPL is compatible with existing rendering engines and we make it available for research purposes.},
journal = {ACM Trans. Graph.},
month = {oct},
articleno = {248},
numpages = {16},
keywords = {soft-tissue, skinning, body shape, blendshapes}
}


@article{b20,
  title={Human3.6M: Large Scale Datasets and Predictive Methods for 3D Human Sensing in Natural Environments},
  author={Catalin Ionescu and Dragos Papava and Vlad Olaru and Cristian Sminchisescu},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  year={2014},
  volume={36},
  pages={1325-1339},
  url={https://api.semanticscholar.org/CorpusID:4244548}
}

@INPROCEEDINGS{b21,
  author={Robinette, K.M. and Daanen, H. and Paquet, E.},
  booktitle={Second International Conference on 3-D Digital Imaging and Modeling (Cat. No.PR00062)}, 
  title={The CAESAR project: a 3-D surface anthropometry survey}, 
  year={1999},
  volume={},
  number={},
  pages={380-386},
  keywords={Anthropometry;Costs;Humans;Area measurement;Volume measurement;Computer aided manufacturing;Europe;Vehicle safety;Automatic control;Mirrors},
  doi={10.1109/IM.1999.805368}}

@ARTICLE{b22,
  author={Tsai, Roger Y. and Huang, Thomas S.},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
  title={Uniqueness and Estimation of Three-Dimensional Motion Parameters of Rigid Objects with Curved Surfaces}, 
  year={1984},
  volume={PAMI-6},
  number={1},
  pages={13-27},
  keywords={Motion estimation;Nonlinear equations;Image analysis;Image sequence analysis;Motion analysis;Image motion analysis;Cameras;Geometry;Singular value decomposition;Matrix decomposition;Dynamic scene analysis;image sequence analysis;motion estimation;motion stereo;optical flow},
  doi={10.1109/TPAMI.1984.4767471}}
@INPROCEEDINGS{b23,
  author={Fang, Qi and Shuai, Qing and Dong, Junting and Bao, Hujun and Zhou, Xiaowei},
  booktitle={2021 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Reconstructing 3D Human Pose by Watching Humans in the Mirror}, 
  year={2021},
  volume={},
  number={},
  pages={12809-12818},
  keywords={Training;Surface reconstruction;Three-dimensional displays;Shape;Pose estimation;Reflection;Pattern recognition},
  doi={10.1109/CVPR46437.2021.01262}}

@article{b24,
author = {Bradski, Gary},
year = {2000},
month = {01},
pages = {},
title = {The openCV library},
volume = {25},
journal = {Dr. Dobb's Journal of Software Tools}
}
@ARTICLE {b25,
author = {Z. Cao and G. Hidalgo and T. Simon and S. Wei and Y. Sheikh},
journal = {IEEE Transactions on Pattern Analysis &amp; Machine Intelligence},
title = {OpenPose: Realtime Multi-Person 2D Pose Estimation Using Part Affinity Fields},
year = {2021},
volume = {43},
number = {01},
issn = {1939-3539},
pages = {172-186},
abstract = {Realtime multi-person 2D pose estimation is a key component in enabling machines to have an understanding of people in images and videos. In this work, we present a realtime approach to detect the 2D pose of multiple people in an image. The proposed method uses a nonparametric representation, which we refer to as Part Affinity Fields (PAFs), to learn to associate body parts with individuals in the image. This bottom-up system achieves high accuracy and realtime performance, regardless of the number of people in the image. In previous work, PAFs and body part location estimation were refined simultaneously across training stages. We demonstrate that a PAF-only refinement rather than both PAF and body part location refinement results in a substantial increase in both runtime performance and accuracy. We also present the first combined body and foot keypoint detector, based on an internal annotated foot dataset that we have publicly released. We show that the combined detector not only reduces the inference time compared to running them sequentially, but also maintains the accuracy of each component individually. This work has culminated in the release of OpenPose, the first open-source realtime system for multi-person 2D pose detection, including body, foot, hand, and facial keypoints.},
keywords = {two dimensional displays;pose estimation;detectors;runtime;kernel;training},
doi = {10.1109/TPAMI.2019.2929257},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month = {jan}
}
@InProceedings{b26,
author="Sturm, Peter
and Bonfort, Thomas",
editor="Narayanan, P. J.
and Nayar, Shree K.
and Shum, Heung-Yeung",
title="How to Compute the Pose of an Object Without a Direct View?",
booktitle="Computer Vision -- ACCV 2006",
year="2006",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="21--31",
abstract="We consider the task of computing the pose of an object relative to a camera, for the case where the camera has no direct view of the object. This problem was encountered in work on vision-based inspection of specular or shiny surfaces, that is often based on analyzing images of calibration grids or other objects, reflected in such a surface. A natural setup consists thus of a camera and a calibration grid, put side-by-side, i.e. without the camera having a direct view of the grid. A straightforward idea for computing the pose is to place planar mirrors such that the camera sees the calibration grid's reflection. In this paper, we consider this idea, describe geometrical properties of the setup and propose a practical algorithm for the pose computation.",
isbn="978-3-540-32432-4"
}
@INPROCEEDINGS{b27,
  author={Varol, Gül and Romero, Javier and Martin, Xavier and Mahmood, Naureen and Black, Michael J. and Laptev, Ivan and Schmid, Cordelia},
  booktitle={2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Learning from Synthetic Humans}, 
  year={2017},
  volume={},
  number={},
  pages={4627-4635},
  keywords={Three-dimensional displays;Shape;Image segmentation;Estimation;Motion segmentation;Solid modeling},
  doi={10.1109/CVPR.2017.492}}
@article{b28,
author = {Kyung, Ho and Jang, Young and Cha, Soon and Jung, Soon},
year = {2003},
month = {01},
pages = {},
title = {3D Reconstruction using Moving Planar Mirror}
}
@INPROCEEDINGS{b29,
  author={Kanbara, M. and Ukita, N. and Kidode, M. and Yokoya, N.},
  booktitle={18th International Conference on Pattern Recognition (ICPR'06)}, 
  title={3D Scene Reconstruction from Reflection Images in a Spherical Mirror}, 
  year={2006},
  volume={4},
  number={},
  pages={874-879},
  keywords={Layout;Image reconstruction;Reflection;Mirrors;Cameras;Reconstruction algorithms;Surface reconstruction;Stereo vision;Calibration;Image sequences},
  doi={10.1109/ICPR.2006.32}}

@INPROCEEDINGS{b30,
  author={Zhong, H. and Sze, W.F. and Hung, Y.S.},
  booktitle={18th International Conference on Pattern Recognition (ICPR'06)}, 
  title={Reconstruction from Plane Mirror Reflection}, 
  year={2006},
  volume={1},
  number={},
  pages={715-718},
  keywords={Mirrors;Reflection;Image reconstruction;Geometry;Cameras;Layout;Computer vision;Stereo vision;Stereo image processing;Reconstruction algorithms},
  doi={10.1109/ICPR.2006.981}}

@INPROCEEDINGS{b31,
  author={Hu, Bo},
  booktitle={2009 Canadian Conference on Computer and Robot Vision}, 
  title={It's All Done with Mirrors: Calibration-and-Correspondence-Free 3D Reconstruction}, 
  year={2009},
  volume={},
  number={},
  pages={148-154},
  keywords={Mirrors;Cameras;Image reconstruction;Reconstruction algorithms;Geometry;Computer vision;Robot vision systems;Calibration;Three dimensional displays;Layout;3-D reconstruction;shape from silhouette;visual hull;camera calibration;catadioptric sensor;mirror},
  doi={10.1109/CRV.2009.29}}

@ARTICLE{b32,
  author={Zhang, Yifu and Wang, Chunyu and Wang, Xinggang and Liu, Wenyu and Zeng, Wenjun},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence}, 
  title={VoxelTrack: Multi-Person 3D Human Pose Estimation and Tracking in the Wild}, 
  year={2023},
  volume={45},
  number={2},
  pages={2613-2626},
  keywords={Three-dimensional displays;Pose estimation;Heating systems;Cameras;Task analysis;Space heating;Noise measurement;3D human pose tracking;volumetric;multiple camera views},
  doi={10.1109/TPAMI.2022.3163709}}

@INPROCEEDINGS {b33,
author = {C. Lassner and J. Romero and M. Kiefel and F. Bogo and M. J. Black and P. V. Gehler},
booktitle = {2017 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
title = {Unite the People: Closing the Loop Between 3D and 2D Human Representations},
year = {2017},
volume = {},
issn = {1063-6919},
pages = {4704-4713},
abstract = {3D models provide a common ground for different representations of human bodies. In turn, robust 2D estimation has proven to be a powerful tool to obtain 3D fits in-the-wild. However, depending on the level of detail, it can be hard to impossible to acquire labeled data for training 2D estimators on large scale. We propose a hybrid approach to this problem: with an extended version of the recently introduced SMPLify method, we obtain high quality 3D body model fits for multiple human pose datasets. Human annotators solely sort good and bad fits. This procedure leads to an initial dataset, UP-3D, with rich annotations. With a comprehensive set of experiments, we show how this data can be used to train discriminative models that produce results with an unprecedented level of detail: our models predict 31 segments and 91 landmark locations on the body. Using the 91 landmark pose estimator, we present state-of-the art results for 3D human pose and shape estimation using an order of magnitude less training data and without assumptions about gender or pose in the fitting procedure. We show that UP-3D can be enhanced with these improved fits to grow in quantity and quality, which makes the system deployable on large scale. The data, code and models are available for research purposes.},
keywords = {three-dimensional displays;solid modeling;shape;two dimensional displays;computational modeling;image segmentation},
doi = {10.1109/CVPR.2017.500},
url = {https://doi.ieeecomputersociety.org/10.1109/CVPR.2017.500},
publisher = {IEEE Computer Society},
address = {Los Alamitos, CA, USA},
month = {jul}
}
@INPROCEEDINGS{b34,
  author={Andriluka, Mykhaylo and Pishchulin, Leonid and Gehler, Peter and Schiele, Bernt},
  booktitle={2014 IEEE Conference on Computer Vision and Pattern Recognition}, 
  title={2D Human Pose Estimation: New Benchmark and State of the Art Analysis}, 
  year={2014},
  volume={},
  number={},
  pages={3686-3693},
  keywords={Estimation;Complexity theory;Joints;Torso;Benchmark testing;Measurement;Training;human pose estimation;performance evaluation},
  doi={10.1109/CVPR.2014.471}}
@InProceedings{b35,
author="Lin, Tsung-Yi
and Maire, Michael
and Belongie, Serge
and Hays, James
and Perona, Pietro
and Ramanan, Deva
and Doll{\'a}r, Piotr
and Zitnick, C. Lawrence",
editor="Fleet, David
and Pajdla, Tomas
and Schiele, Bernt
and Tuytelaars, Tinne",
title="Microsoft COCO: Common Objects in Context",
booktitle="Computer Vision -- ECCV 2014",
year="2014",
publisher="Springer International Publishing",
address="Cham",
pages="740--755",
abstract="We present a new dataset with the goal of advancing the state-of-the-art in object recognition by placing the question of object recognition in the context of the broader question of scene understanding. This is achieved by gathering images of complex everyday scenes containing common objects in their natural context. Objects are labeled using per-instance segmentations to aid in precise object localization. Our dataset contains photos of 91 objects types that would be easily recognizable by a 4 year old. With a total of 2.5 million labeled instances in 328k images, the creation of our dataset drew upon extensive crowd worker involvement via novel user interfaces for category detection, instance spotting and instance segmentation. We present a detailed statistical analysis of the dataset in comparison to PASCAL, ImageNet, and SUN. Finally, we provide baseline performance analysis for bounding box and segmentation detection results using a Deformable Parts Model.",
isbn="978-3-319-10602-1"
}
@INPROCEEDINGS{b36,
  author={Fieraru, Mihai and Zanfir, Mihai and Pirlea, Silviu Cristian and Olaru, Vlad and Sminchisescu, Cristian},
  booktitle={2021 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={AIFit: Automatic 3D Human-Interpretable Feedback Models for Fitness Training}, 
  year={2021},
  volume={},
  number={},
  pages={9914-9923},
  keywords={Training;Visualization;Solid modeling;Three-dimensional displays;Shape;Real-time systems;Sensors},
  doi={10.1109/CVPR46437.2021.00979}}

@Inbook{b37,
author="Sminchisescu, Cristian",
editor="Rosenhahn, Bodo
and Klette, Reinhard
and Metaxas, Dimitris",
title="3D Human Motion Analysis in Monocular Video: Techniques and Challenges",
bookTitle="Human Motion: Understanding, Modelling, Capture, and Animation",
year="2008",
publisher="Springer Netherlands",
address="Dordrecht",
pages="185--211",
abstract="Extracting meaningful 3D human motion information from video sequences is of interest for applications like intelligent human--computer interfaces, biometrics, video browsing and indexing, virtual reality or video surveillance. Analyzing videos of humans in unconstrained environments is an open and currently active research problem, facing outstanding scientific and computational challenges. The proportions of the human body vary largely across individuals, due to gender, age, weight or race. Aside from this variability, any single human body has many degrees of freedom due to articulation and the individual limbs are deformable due to moving muscle and clothing. Finally, real-world events involve multiple interacting humans occluded by each other or by other objects and the scene conditions may also vary due to camera motion or lighting changes. All these factors make appropriate models of human structure, motion and action difficult to construct and difficult to estimate from images. In this chapter we give an overview of the problem of reconstructing 3D human motion using sequences of images acquired with a single video camera. We explain the difficulties involved, discuss ways to address them using generative and discriminative models and speculate on open problems and future research directions.",
isbn="978-1-4020-6693-1",
doi="10.1007/978-1-4020-6693-1_8",
url="https://doi.org/10.1007/978-1-4020-6693-1_8"
}

@INPROCEEDINGS{b38,
  author={Goutsu, Yusuke and Inamura, Tetsunari},
  booktitle={2021 IEEE International Conference on Robotics and Automation (ICRA)}, 
  title={Linguistic Descriptions of Human Motion with Generative Adversarial Seq2Seq Learning}, 
  year={2021},
  volume={},
  number={},
  pages={4281-4287},
  keywords={Training;Learning systems;Gradient methods;Monte Carlo methods;Stochastic processes;Reinforcement learning;Linguistics},
  doi={10.1109/ICRA48506.2021.9561519}}

@article{b39,
  title={Statistical mutual conversion between whole body motion primitives and linguistic sentences for human motions},
  author={Wataru Takano and Yoshihiko Nakamura},
  journal={The International Journal of Robotics Research},
  year={2015},
  volume={34},
  pages={1314 - 1328},
  url={https://api.semanticscholar.org/CorpusID:38292554}
}
@book{b40,
author = {Prince, Simon J. D.},
title = {Computer Vision: Models, Learning, and Inference},
year = {2012},
isbn = {1107011795},
publisher = {Cambridge University Press},
address = {USA},
edition = {1st},
abstract = {This modern treatment of computer vision focuses on learning and inference in probabilistic models as a unifying theme. It shows how to use training data to learn the relationships between the observed image data and the aspects of the world that we wish to estimate, such as the 3D structure or the object class, and how to exploit these relationships to make new inferences about the world from new image data. With minimal prerequisites, the book starts from the basics of probability and model fitting and works up to real examples that the reader can implement and modify to build useful vision systems. Primarily meant for advanced undergraduate and graduate students, the detailed methodological presentation will also be useful for practitioners of computer vision. - Covers cutting-edge techniques, including graph cuts, machine learning, and multiple view geometry. - A unified approach shows the common basis for solutions of important computer vision problems, such as camera calibration, face recognition, and object tracking. - More than 70 algorithms are described in sufficient detail to implement. - More than 350 full-color illustrations amplify the text. - The treatment is self-contained, including all of the background mathematics. - Additional resources at www.computervisionmodels.com.}
}

@INPROCEEDINGS{b41,
  author={Beckouche, Simon and Leprince, Sébastien and Sabater, Neus and Ayoub, François},
  booktitle={2011 IEEE International Conference on Computer Vision Workshops (ICCV Workshops)}, 
  title={Robust outliers detection in image point matching}, 
  year={2011},
  volume={},
  number={},
  pages={180-187},
  keywords={Transforms;Estimation;Kernel;Robustness;Mathematical model;Accuracy;Noise},
  doi={10.1109/ICCVW.2011.6130241}}

@Inbook{Zhang2014,
author="Zhang, Zhengyou",
editor="Ikeuchi, Katsushi",
title="Epipolar Geometry",
bookTitle="Computer Vision: A Reference Guide",
year="2014",
publisher="Springer US",
address="Boston, MA",
pages="247--258",
isbn="978-0-387-31439-6",
doi="10.1007/978-0-387-31439-6_128",
url="https://doi.org/10.1007/978-0-387-31439-6_128"
}

